Adaptive Depth Networks with Skippable Sub-Paths

Predictable adaptation of network depths can be an effective way to control inference latency and meet the resource condition of various devices. However, previous adaptive depth networks do not provide general principles and a formal explanation on why and which layers can be skipped, and, hence, their approaches are hard to be generalized and require long and complex training steps. In this paper, we present a practical approach to adaptive depth networks that is applicable to various networks with minimal training effort. In our approach, every hierarchical residual stage is divided into two sub-paths, and they are trained to acquire different properties through a simple self-distillation strategy. While the first sub-path is essential for hierarchical feature learning, the second one is trained to refine the learned features and minimize performance degradation if it is skipped. Unlike prior adaptive networks, our approach does not train every target sub-network in an iterative manner. At test time, however, we can connect these sub-paths in a combinatorial manner to select sub-networks of various accuracy-efficiency trade-offs from a single network. We provide a formal rationale for why the proposed training method can reduce overall prediction errors while minimizing the impact of skipping sub-paths. We demonstrate the generality and effectiveness of our approach with convolutional neural networks and transformers.

==> checklist.tex <==

\section*{NeurIPS Paper Checklist}


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: \justificationTODO{}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    In Section \ref{sec:on-device-perf},
    Figure \ref{fig:exp-train-test}-(b) highlights 
    both the advantage and a limitation of our approach. 
    While the compared adaptation method, e.g., width scaling,
    provides a wider FLOPs adaptation range, 
    our approach of adapting depths has a more limited adaptation range. 
    As shown in Figure \ref{fig:skippableratio},
    this limitation stems from the fact that maintaining certain depths
    in mandatory sub-paths is crucial for effective inference.
    To achieve further FLOPs scaling, we may need to explore synergies with other adaptation dimensions, such as adjusting network widths \cite{yu2018slimmable} and input resolutions \cite{yang2020resolution}, along with our depth adaptation method. 
    We leave this as our future work.

    In Section \ref{sec:training-time}, we mention that the prior adaptive networks we selected for the comparison of training time may seem outdated. 
    While we acknowledge the importance of recent literature, there are limited works that closely align with our specific approach. 
    For instance, research on adaptive networks in the context of CNNs is not very active recently. 
    Research specifically addressing the reduction of training time for adaptive networks is even further scarce. This scarcity of recent research may be attributed to the impracticality of prior adaptive networks, which is characterized by lengthy and complex training procedures and relatively low inference performance.
    This impracticality of prior adaptive networks 
    is the major motivation for our research.
    For vision transformers, there are some studies on dynamic networks and our paper also cites some of these relevant studies in Table \ref{table:imagenet-sota}. 
    However, their emphasis tends to be on improving accuracy rather than reducing training time. We believe that the scarcity of recent prior research in this area implies that our study introduces a novel direction in this field.


    

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section \ref{sec:theory} provides formal
    analysis of our work. 

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide source codes and pretrained weights as supplementary material. 
    The source codes includes default settings, e.g., hyperameters,
    used in the evaluation.
    Further, we provide more detailed experiment settings in Appendix \ref{sec:arch-detail}.
        
    
\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide source codes and pretrained weights as supplementary material. They will be available in github 
    shortly for open access.
    
\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section \ref{sec:exp_detection} and 
    Appendix \ref{sec:arch-detail} provide details of the evaluation.
    Further the source codes includes default settings, e.g., hyperameters,
    used in the evaluation.
    
\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use ImageNet and COCO datasets for experiments. 
    Training models with these large datasets requires too much computing resources to obtain meaningful errorbars. 
    
\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In the experiments, we mention what kinds of 
    computing resource is used. 
    For example, in Section \ref{sec:exp}, we mention that RTX 4090s, 3090s were used for training.
    In Section \ref{sec:on-device-perf}, we mention that Nvidia Jetson Orin Nano was used to evaluate on-device performance.
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.

\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    We can hardly think of negative societal impact of our work
    since the goal of this work is to make deep learning training and inference more energy-efficient. Our approach not only accelerates model development but also contributes to sustainability efforts.
       
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.

\end{enumerate}


==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


